Mastery Guided Non-parametric Clustering to Scale-up Strategy Prediction

Predicting the strategy (sequence of concepts) that a student is likely to use in problem-solving helps Adaptive Instructional Systems (AISs) better adapt themselves to different types of learners based on their learning abilities. This can lead to a more dynamic, engaging, and personalized experience for students. To scale up training a prediction model (such as LSTMs) over large-scale education datasets, we develop a non-parametric approach to cluster symmetric instances in the data. Specifically, we learn a representation based on Node2Vec that encodes symmetries over mastery or skill level since, to solve a problem, it is natural that a student's strategy is likely to involve concepts in which they have gained mastery. Using this representation, we use DP-Means to group symmetric instances through a coarse-to-fine refinement of the clusters. We apply our model to learn strategies for Math learning from large-scale datasets from MATHia, a leading AIS for middle-school math learning. Our results illustrate that our approach can consistently achieve high accuracy using a small sample that is representative of the full dataset. Further, we show that this approach helps us learn strategies with high accuracy for students at different skill levels, i.e., leveraging symmetries improves fairness in the prediction model.

==> sections/results-interaction.tex <==
\begin{figure*}
\centering
\subfigure[]{\scalebox{0.6}{\begin{tikzpicture}
    \begin{axis}[
    	title={Results for BA08},
    	xlabel={Attention Threshold},
    	ylabel={Test Accuracy(\%)},
    	xmin=0, xmax=0.35,
    	ymin=60, ymax=90,
    	xtick={0.05, 0.10, 0.15, 0.20, 0.25, 0.30},
    	ytick={65, 70, 75, 80, 85, 90},
    	legend pos=south east,
    	ymajorgrids=true,
    	xmajorgrids=true,
    	grid style=dashed,
    	legend style={nodes={scale=0.55, transform shape}}
    ]
    
    \addplot[color=orange, mark=square, smooth]
    	table[x=prune, y=acc] {attn-samp-bridge-3k.dat};
    \addlegendentry{3k samples}
    
    \addplot[color=red, mark=x, smooth]
    	table[x=prune, y=acc] {attn-samp-bridge-6k.dat};
    \addlegendentry{6k samples}
    
    \addplot[color=blue, mark=o, smooth]
    	table[x=prune, y=acc] {attn-samp-bridge-20k.dat};
    \addlegendentry{20k samples}
    
    \addplot[color=brown, mark=triangle, smooth]
    	table[x=prune, y=acc] {attn-samp-bridge-40k.dat};
    \addlegendentry{40k samples}
    
    \end{axis}
\end{tikzpicture}}}
\quad
\subfigure[]{\scalebox{0.6}{\begin{tikzpicture}
    \begin{axis}[
    	title={Results for CL19},
    	xlabel={Attention Threshold},
    	ylabel={Test Accuracy(\%)},
    	xmin=0, xmax=0.35,
    	ymin=60, ymax=90,
    	xtick={0.05, 0.10, 0.15, 0.20, 0.25, 0.30},
    	ytick={65, 70, 75, 80, 85, 90},
    	legend pos=south east,
    	ymajorgrids=true,
    	xmajorgrids=true,
    	grid style=dashed,
    	legend style={nodes={scale=0.55, transform shape}}
    ]
    
    \addplot[color=orange, mark=square, smooth]
    	table[x=prune, y=acc] {attn-samp-mathia-3k.dat};
    \addlegendentry{3k samples}
    
    \addplot[color=red, mark=x, smooth]
    	table[x=prune, y=acc] {attn-samp-mathia-6k.dat};
    \addlegendentry{6k samples}
    
    \addplot[color=blue, mark=o, smooth]
    	table[x=prune, y=acc] {attn-samp-mathia-20k.dat};
    \addlegendentry{20k samples}
    
    \addplot[color=brown, mark=triangle, smooth]
    	table[x=prune, y=acc] {attn-samp-mathia-40k.dat};
    \addlegendentry{40k samples}
    
    \end{axis}
\end{tikzpicture}}}
\quad
\subfigure[]{\scalebox{0.8}{\begin{tikzpicture}
    \begin{axis} [ybar, 
        ymin=50, 
        ymax=100, 
        ylabel={Accuracy (\%)}, 
        xlabel={Student Performance Groups (\%)},
        symbolic x coords={0-30, 30-50, 50-70, 70-90, 90-100},
        legend pos=south east,
        legend style={nodes={scale=0.75, transform shape}},
        nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\tiny, color=black}
        ]

    \addplot [black, fill] coordinates {(0-30,66.77) (30-50,74.15) (50-70,74.68) (70-90,81.1) (90-100,78.9)};
    \addplot [cyan, fill] 
    coordinates {(0-30,84.61) (30-50,88.61) (50-70,88.75) (70-90,88.47) (90-100, 90.38)};
    \addplot [orange, fill] coordinates {(0-30,90.84) (30-50,92.21) (50-70,93.33) (70-90,91.14) (90-100,92.71)};
    
    
    \legend {NS, SS, SS + MS};
    
    \end{axis}
\end{tikzpicture}}}
% \quad
% \subfigure[]{\scalebox{0.6}{\begin{tikzpicture}
%     \begin{axis} [ybar, 
%         ymin=50, 
%         ymax=100, 
%         ylabel={Accuracy (\%)}, 
%         xlabel={Student Performance Groups (\%)},
%         symbolic x coords={0-30, 30-50, 50-70, 70-90, 90-100},
%         legend pos=north west,
%         legend style={nodes={scale=0.75, transform shape}},
%         nodes near coords,
%         nodes near coords align={vertical},
%         nodes near coords style={font=\tiny, color=black}
%         ]
    
%     \addplot [cyan, fill] 
%     coordinates {(0-30,88.2) (30-50,91.35) (50-70,94.32) (70-90,90.47) (90-100,92.13)};
%     \addplot [orange, fill] coordinates {(0-30,80.8) (30-50,83.1) (50-70,83.4) (70-90,84.5) (90-100,82.9)};
    
%     \legend {Train, Test};
    
%     \end{axis}
% \end{tikzpicture}}}

\caption{(a) and (b) show the influence of the attention threshold for mastery atoms. The x-axis shows the threshold we use on attention values to compute the mastery atoms and the y-axis shows the test accuracy obtained when we set this threshold. (c) shows accuracy for different groups of students (based on their performance). The x-axis denotes different ranges of \%s, where a range $a-b$ denotes that students in this group got $>a$ and $<b$ steps correct in their first attempt. The y-axis shows accuracy over the groups. As seen here, our model was fair where the accuracy is invariant to performance-based groups and outperforms the model without mastery.}
\label{fig:pruning}
\end{figure*}

%Illustrating the influence of attention in strategies. The x-axis illustrates the \% of formulas related to the original KCs that are removed (based on an attention threshold) while re-learning the embedding for the final strategy prediction model.
